Towards the Usage of MBT at ETSI

In 2012 the Specialists Task Force (STF) 442 appointed by the European Telcommunication Standards Institute (ETSI) explored the possibilities of using Model Based Testing (MBT) for test development in standardization. STF 442 performed two case studies and developed an MBT-methodology for ETSI. The case studies were based on the ETSI-standards GeoNetworking protocol (ETSI TS 102 636) and the Diameter-based Rx protocol (ETSI TS 129 214). Models have been developed for parts of both standards and four different MBT-tools have been employed for generating test cases from the models. The case studies were successful in the sense that all the tools were able to produce the test suites having the same test adequacy as the corresponding manually developed conformance test suites. The MBT-methodology developed by STF 442 is based on the experiences with the case studies. It focusses on integrating MBT into the sophisticated standardization process at ETSI. This paper summarizes the results of the STF 442 work.

==> eptcsdata.tex <==
\providecommand{\firstpage}{30}
\providecommand{\publicationstatus}{A. Petrenko, H. Schlingloff (Eds.): Eighth Workshop on\\ Model-Based Testing (MBT 2013)\\
EPTCS 111, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.111.3}{10.4204/EPTCS.111.3}}
\pdfoutput=1

